Learning Diverse Options via InfoMax Termination Critic

We consider the problem of autonomously learning reusable temporally extended actions, or options, in reinforcement learning. While options can speed up transfer learning by serving as reusable building blocks, learning reusable options for unknown task distribution remains challenging. Motivated by the recent success of mutual information (MI) based skill learning, we hypothesize that more diverse options are more reusable. To this end, we propose a method for learning termination conditions of options by maximizing MI between options and corresponding state transitions. We derive a scalable approximation of this MI maximization via gradient ascent, yielding the InfoMax Termination Critic (IMTC) algorithm. Our experiments demonstrate that IMTC significantly improves the diversity of learned options without extrinsic rewards combined with an intrinsic option learning method. Moreover, we test the reusability of learned options by transferring options into various tasks, confirming that IMTC helps quick adaptation, especially in complex domains where an agent needs to manipulate objects.

==> appendices/a-chain.tex <==
\section{InfoMax Options in Deterministic Chain}
\label{appendix:chain}

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{6.8cm}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case1-1.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case1-2.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{6.8cm}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-1.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-2.pdf}
  \end{subfigure}
  \caption{
    Two instances of InfoMax options in the four-state deterministic chain.
    \textbf{Left:} Options are diverse, but all state transitions per option are one-step.
    \textbf{Right:} Options enable relatively long state transitions, but intra-option policies are the same in some states.
  }
  \label{figure:opt2-chain}
\end{figure}

To illustrate the limitation of infomax options, we analyzed a toy four-state \textit{deterministic chain} environment, which has four states and two deterministic actions (left and right) per each state.
Deriving the exact solution is difficult, and thus, we only considered deterministic options with a minimum $H(X_f|x_s, O)$ and maximize $H(X_f|x_s)$.
Among the multiple solutions, we show two interesting deterministic infomax options when $|\Op| = 2$ in \Cref{figure:opt2-chain}.
The left options enable diverse behaviors per state, although they fail to capture long-term behaviors that are generally favorable in the literature (e.g., \citet{Mann2015AVI}).
Conversely, the right options enable relatively long, two- or three-step transitions while policies are the same in three states.
Furthermore, we can see that the two options form a small loop between the leftmost two states.
As this example shows, a major caveat of this MI-based approximation of diversity is the inability to consider the distance between states.
Therefore, neighboring states can be assigned to different groups, resulting in short options that are often undesirable.
While we do not observe such short options in \Cref{section:experiments: intrinsic} with Euclidian state spaces, this can still be problematic in general.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{6.8cm}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-1.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-2.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt3-case1-3.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{6.8cm}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-1.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt2-case2-2.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt3-case1-3.pdf}
    \includegraphics[width=6.5cm]{figures/chains/opt4-case1-4.pdf}
  \end{subfigure}
  \caption{
     InfoMax options in the four state deterministic chain.
     \textbf{Left: } With three options.
     \textbf{Right: } With four options.
  }
  \label{figure:opt3-4-chain}
\end{figure}
\Cref{figure:opt3-4-chain} shows deterministic infomax options when $|\Op| = 3$ and when $|\Op| = 4$.
Among multiple solutions, we selected options with an absorbing state per option (i.e., $\bo(x) = 1.0$ for only one $x$), which are partially the same as the right options in \Cref{figure:opt2-chain}.
With four options, $\Pr(x_f|x_s) = 0.25$ for all $x_f$ and $x_s$, thus $H(X_f|x_s)$ is the maximum for all $x_s$.
This example suggests that we need as many options as the number of states to ensure that the short-cycle problem would not happen.
